Evaluating Multimodal Interaction of Robots Assisting Older Adults

We outline our work on evaluating robots that assist older adults by engaging with them through multiple modalities that include physical interaction. Our thesis is that to increase the effectiveness of assistive robots: 1) robots need to understand and effect multimodal actions, 2) robots should not only react to the human, they need to take the initiative and lead the task when it is necessary. We start by briefly introducing our proposed framework for multimodal interaction and then describe two different experiments with the actual robots. In the first experiment, a Baxter robot helps a human find and locate an object using the Multimodal Interaction Manager (MIM) framework. In the second experiment, a NAO robot is used in the same task, however, the roles of the robot and the human are reversed. We discuss the evaluation methods that were used in these experiments, including different metrics employed to characterize the performance of the robot in each case. We conclude by providing our perspective on the challenges and opportunities for the evaluation of assistive robots for older adults in realistic settings.

==> Task_Network.tex <==
\section{Multimodal Interaction Manager}
\label{Task Network}



Our goal is to develop a multimodal interaction manager, as in Fig.~\ref{fig:HRI}, that allows a robot to collaborate with a human partner on a task using spoken utterances and physical actions. To this end, we designed data-driven models for each subtask, which we describe in detail in this section. using the annotated data described above 


\iffalse
\begin{enumerate}
\item \textit{Det($O_{T}$)}: determining the object type that needs to be found. 
\item \textit{Det($L$)}: determining the potential location of the object. %In other words, this subtask recognizes the potential location for the requested object.  
\item \textit{Open}: open/check the determined location in the previous subtask.
\item \textit{Det($O$)}: looking for the object, and if it is found confirm with the elder. If the object is not found at this step, it loops back to the previous subtasks to modify the parameters.
\end{enumerate}
\fi


We first establish a representation of multimodal actions performed by the human that is observed and interpreted by the robot in the Interpretation Module. We define a vector containing the following features for each observed move:

\begin{enumerate}
    \item whether or not an object type is uttered
    \item the DA tag
    \item whether or not a location is uttered
    \item whether or not an H-O action is performed 
    \item whether or not a pointing gesture is performed 
\end{enumerate}
Each of the features is binary, except the DA tag, which is categorical. For observed moves that are only physical actions (no utterances), the DA tag feature can be empty. Then given an observed human move as a vector, the \componentname{} should be able to produce an appropriate responding move (also as a vector).


The challenge in modeling each subtask is that because there are two agents (ELD and HEL), the fact that each agent's actions affect the other's actions must be considered. Here, we propose to model this problem using an \subtaskname{} (\subtaskacro{}), in which both agents' states and actions are incorporated in a single graph, and transitions are triggered by action vectors. Fig.~\ref{fig:task_network} shows an \subtaskacro{} for \textit{Det($L$)}, where blue nodes represent states in which HEL should perform the next move, red nodes for states in which ELD should perform the next move, and white nodes for end states.
%Note that the network in Fig.~\ref{fig:task_network} is condensed in that some values of the vectors are (*), which denotes that any value can fill that feature.


Using the segmented data in the corpus, we derived \subtaskacroplural{} for each subtask and counted frequencies of possible paths through the \subtaskacroplural{}, i.e., possible sequences of moves in each subtask. The frequencies determined the probability of taking each path, which was used to model the stochastic behavior of interactions. The \componentname{} then uses these models to navigate each subtask, deciding which action to perform next given an interpreted action. We note that the purpose of \subtaskacroplural{} in our framework then is to help estimate the current state of the human participant given their actions, as well as plan the next robot move from the resulting robot state.

To better illustrate this, we will walk through an example using Fig.~\ref{fig:task_network}. Suppose the robot (as HEL) is in state $s_0$. It can select one of the possible actions using the calculated probabilities from the training data. Suppose the action [1, Query-w, 0, 0, 0] is selected (the robot asks a question about where the object is located). 
%Then, the robot estimates possible human states and waits for the human partner's observed move vector. 
The human is then estimated to be in state $s_2$, and the robot's next state depends on the vector of observations from the human. If the human answers the robot's question with an utterance containing a location name -- [0, Reply-w, 1, 0, 0] -- the robot chooses $s_3$ or $s_6$, again based on the probabilities from the training data.

 

When more than one human state is possible after a robot's action, a state is chosen by comparing the observed human action with all of the possible human actions from the set of estimated states. The state with the closest matching action (defined by matching feature values, with preference given to matching DA tags) is selected as the most likely human state. If no action is reasonably similar to the observed action (here, defined as no matching DA tags), then the robot asks the user to repeat their action, after which another failure would result in stochastically choosing the human state.

When the end of a subtask is reached, the next state depends on the next subtask, which depends on whether or not the subtask was completed, e.g., whether or not the \textit{Det($L$)} interaction ended with a location determined. If the subtask is completed, then the next subtask is given in the hierarchical task decomposition; otherwise, the subtask must be repeated. Note that \textit{Det($O$)} is completed when an object is determined to be the target object or when an object is determined to not be the target object. In the former case, the \textit{Find} task is complete, whereas in the latter case, a new object or location must be chosen. For each subtask, either ELD or HEL can initiate the interaction. Thus, for each subtask, there are two \subtaskacro{} components.
%, except for \textit{Det(O)} -- in this subtask, HEL needs to recognize the object and compare it with the target object, so HEL always initiates this subtask.
%Furthermore, the framework can update the needed parameters in all the subtasks if it is needed. For example, the elder can change the target object after proceeding in \textit{Det(L)} subtask. 

Because the \textit{Find} task is decomposed hierarchically into subtasks, and each subtask is modeled by an \subtaskacro{}, we consider our \componentname{} a \modelname{} (\modelacro{}). As desired, this unified framework integrates physical actions (both pointing and H-O) and language while maintaining the state of the interaction to move towards completing the goal and provide appropriate responses. Another advantage of this framework is in its flexibility: once the model is generated, the robot can take on any role\OUT{the role of either HEL or ELD} and interact with the human accordingly. 
%BDE: if you put the role of ELD one would say "and why would the robot do that"? one would have to explain that the HEL can be active as well etc. 

%We also note that the proposed architecture is general enough that it can be easily extended to more complex activities such as collaborative manipulation \cite{noohi2016model} and object handover \cite{parastegari2016fail,parastegari2018failure}. 
We also note that the proposed architecture is general enough that it can be applied to other task-oriented multimodal human-robot interactions, such as collaborative manipulation \cite{noohi2016model} and object handover \cite{parastegari2016fail,parastegari2018failure}, by decomposing the tasks analogously and defining appropriate action vectors.
While the topology of each \subtaskacro{} was derived from the data by human inspection for expediency in this work, automating this process using well-established techniques similar to those used for learning Markov models \cite{murphy2012machine} will be the subject of future work.
